An Adaptive Orthogonal Convolution Scheme for Efficient and Flexible CNN Architectures

Orthogonal convolutional layers are valuable components in multiple areas of machine learning, such as adversarial robustness, normalizing flows, GANs, and Lipschitz-constrained models. Their ability to preserve norms and ensure stable gradient propagation makes them valuable for a large range of problems. Despite their promise, the deployment of orthogonal convolution in large-scale applications is a significant challenge due to computational overhead and limited support for modern features like strides, dilations, group convolutions, and transposed convolutions. In this paper, we introduce AOC (Adaptative Orthogonal Convolution), a scalable method that extends a previous method (BCOP), effectively overcoming existing limitations in the construction of orthogonal convolutions. This advancement unlocks the construction of architectures that were previously considered impractical. We demonstrate through our experiments that our method produces expressive models that become increasingly efficient as they scale. To foster further advancement, we provide an open-source python package implementing this method, called Orthogonium ( https://github.com/deel-ai/orthogonium ) .

==> flash_bcop/parts/legacy.tex <==
\thib{This is legacy writing (old notes)}

\paragraph{Properties of \Bconv{}:}


\red{ton image est pas mal ca pourrait fa   ire un beau tableau probablement en annexe par contre, et j'ai essayé de faire le travail de sous quelles hypothese c'est valable pour les premiers mais ca fait long.}
    
    \paragraph{OLD Notations:}
    \begin{itemize}
        \item $\mathcal{K}_{c_o,c_i,k_1,k_2}$ the set of kernels. Since we can add zero padding without affecting the underlying convolution we can denote $\mathcal{K}$ the set of convolution with infinite support. 
        \item $A \mathbconv B: {K}_{c_o,c,l_1,l_2} \times {K}_{c,c_i,k_1,k_2} \rightarrow {K}_{c_o,c_i,(k_1+l_1-1),(k_2+l_2-1)}$ denote the block convolution.\red{Franck : j'aurais mis :
"i.e. the equivalent kernel of the composition of the two convolutions.", mais vu qu'apres tu parle du fait que ca ne marche pas en zero padding c'est peut etre pas le cas. En tout cas ca manque de definition claire.}
        \item  Tensor representing kernel are capitalized
        \item their shape is assumed to be $k_A \times k_A \times c_{in} \times c{out}$. \red{pourquoi au dessus c'etait $c_o,c_i,k_1,k_2$?}
        \item Vectors are written lower case (ie. $x$), it's shape is assumed to be $ b \times c_{in} \times i_w \times i_h $, \red{where $b$ is the batch size.}
    \end{itemize}

    \paragraph{Properties of block convolution:}This operation is associative: 
    \[ A \mathbconv (B \mathbconv C) = (A \mathbconv B ) \mathbconv C \]
    However it is not commutative\red{(since composition of convolution is not)}:
    \[ A \mathbconv B \neq B \mathbconv A \]
    It is a linear application:
    \[ \lambda_1 A * x + \lambda_2 B * x = (\lambda_1 A + \lambda_2 B) * x \]
    We also have, for circular convolutions:
    \[ (A \mathbconv B) * x = A * ( B * x))  \]
    This can be trivially extended to convolutions with padding "valid". However, this is not true when padding is "same", since the composition should include the padding operation (the writing of the $\mathbconv$ operator for convolutions with constant padding is certainly possible, but we leave this for future works). % by adding 0 padding whose size is $\lfloor k / 2 \rfloor + 1$ such that circular padding get ignored.

    % \paragraph{Activation functions:}
    % For most activation functions there is no closed form for fusing, however, the specific case of ReLU admits a closed form:
    % \begin{align*}
    %     A * ReLU( B * x ) =& (A \mathbconv ReLU(B)) * ReLU(x) \\
    %     & + (A \mathbconv -ReLU(-B)) * -ReLU(-x)
    % \end{align*}
    % This formula can be applied to several blocks used in famous architectures: for instance, it can be used to merge depth-wise and point-wise convolutions even when there is an activation between them. Recursion can be used to extend this notation to more than two layers, but this approach makes the model exponentially larger as we reduce depth. It is indeed worth noting that, when the network is the interleave of ReLU and convolutions, we can assume the $x$ only contains positive values, hence simplifying the closed form.
\red{ajouter $(A\mathbconv  B)^T = B^T\mathbconv A^T$ et mettre un warning sur le fait que ce n'est pas le kernel qui est tranposé. + ajout de stride $A_s\mathbconv B$}

    % \sout{\paragraph{Field algebra} \red{J'ai discuté avec Louis il convient que c'est une connerie et ne connait pas de nom qd toutes elements ne peuvent pas etre 'multipliés'}it defines a field \red{associative} algebra $(A, +, ., \mathbconv)$. ie. $(A,+,.)$ is a vector space. $A \mathbconv A \rightarrow A$ and $\mathbconv$ is bi-linear. Note: $\mathbconv$ is a group action. Todo: explcit e the kernel of the identity convolution.
    % \red{verifier que dans fiel algebra il n'y a pas besoin d'avoir tout A et B $A\mathbconv B$ existe.Ici c'est faux}}
    % \paragraph{Remark:} The block operation $ \mathbconv $ applied to kernels is equivalent to implicitly multiplying the Toeplitz matrices that represent the linear operation defined by their kernel. 

    % \paragraph{Stride and dilation:} \textbf{Stride and dilation are not handled yet but this can certainly be implemented as for "same" padding.}

    \paragraph{Orthogonal matrices}

        A row orthogonal is a matrix such that $ WW^t = I $ and a column orthogonal is a matrix such that $ W^tW = I $. Trivially the transpose of a row-orthogonal matrix is a column orthogonal matrix and vice-versa.
        
        \paragraph{Row/Columns masking of a Row/columns orthogonal matrix:} If we remove rows of a row-orthogonal matrix, the resulting matrix is still a row orthogonal matrix, Same goes for a column orthogonal matrix.

        \paragraph{Composition of row/column orthogonal matrices:} The product of row (resp columns) orthogonal matrices is a row (resp. columns) orthogonal matrix. However, the product of a row ortho with a col orth is neither row nor col orthogonal.

        \paragraph{remark about convolution and row/column orthogonality:} The shape of the Toeplitz matrix of a convolution must not be confused with the shape of its kernel. Especially the Toeplitz matrix has more rows than columns if $ c_i * s^2 \geq c_o $. \red{citer existence}% A convolution is row/column orthogonal if the Toeplitz matrix that represents its linear application is row/column orthogonal. 

\red{A voir si interet:  complexite en terme de nombre de parametre cxcxk et comparer avec SC-fac ....} 

\section{Turbocharging old methods}

    \subsection{Advantages and limitations of previous methods}

    On one side we have RKO that comes with its advantage: good handling of channel change and efficient striding, and drawbacks: it is not orthogonal when stride $\neq$ kernel size. On the other side, methods such as BCOP, SOC, ECO, LOT and Cayley handle any kernel size but channel change (when $c_i \neq c_o$) is handled with padding/channel dropping, and striding is emulated in a way that makes the convolution more costly than when striding is not applied.

    \begin{theorem}[RKO is orthogonal when stride=kernel size]
        Proof sketch: this is equivalent with applying invertible downsampling and a 1x1 conv. The 1x1 conv consists in a linear combination of the $kxkxc_i$ channels. The resulting toeplitz matrix has then a block diagonal structure. When each block is orthogonal, the whole matrix is orthogonal. The orthogonalization of each block is exactly the operation done by RKO. 
    \end{theorem}

    We make use of our ability to fuse kernels to make the drawbacks of each approach cancel out.

    \subsection{Extending parametrizations to channel change, striding and groups}

        \paragraph{Handling channels change}
            \begin{theorem}[Composition of orthogonal convolutions]\label{thm_comp}
            the composition of two row (resp column) orthogonal convolutions is a row (resp column)  orthogonal convolution. sketch of the proof: we look at the Toeplitz matrix of the orthogonal convolution, those are rotation matrices so the product of these is still a rotation matrix, ie. an orthogonal convolution.
            \end{theorem}

            
            Under some conditions, we can extend this lemma to non-square matrices. The requirement is that the underlying toeplitz matrices must have monotonic rank (ie. $A \in \mathbb{R}^{m_1\times m_2}, B \in \mathbb{R}^{m_2\times m_3}$ with $m_1 \leq m_2 \leq m_3$ or $m_3 \leq m_2 \leq m_1$. Sketch of the proof: We need to show that we can decompose any non-square orthogonal matrix as an orthogonal projection matrix and an orthogonal square matrix with a lower rank.
            Thanks to this property, following the strategy depicted in \cite{senderovich2022towards} we can then write our convolution in two parts: 
            A) when $c_i > c_o $ a 1x1 RKO convolution that reduces channels from $c_i$ to $c_o$ followed by a kxk bcop convolution with the same amount of input and output channels.
            B) when $c_i < c_o$ we start with the bcop conv and follow with the 1x1 conv.
            by doing so we can ensure that bcop parametrization is done on $min(c_i,c_o)$ which is more efficient. The bloc convolution $\mathbconv$ allows us to fuse the kernels to create a single kxk kernel.

        \paragraph{Handling strides}

        \begin{theorem}[bloc convolution and striding]\label{thm_stride} when the first convolution uses circular padding and the second convolution uses striding. We can fuse the kernel and apply striding on the resulting conv. Sketch of the proof: unfold the summation, we find the summation of convolution using the fused kernel and applied with striding. 
        \end{theorem}

        Then we can make use of this to build orthogonal conv with striding: since RKO is orthogonal when kernel size = stride, we can combine a bcop conv with kernel size (k-stride + 1) with a rko conv with kernel size = stride. The resulting fused kernel is a kxk with stride s. Again we combined 2 orthogonal convs so the resulting convolution is orthogonal, this is a composition of \ref{thm_comp} and \ref{thm_stride}.

        \paragraph{Handling transposed convolutions} 
        
        By definition, the transposed convolution implements the implicit product with the transpose of the Toeplitz matrix defined by the kernel. Hence all orthogonal methods that have 1. explicit kernel and 2. native striding, can reuse the kernel directly in the conv transpose to build an orthogonal conv transpose.

        \paragraph{Handling groups} TODO. Recall proof: a block diagonal matrix if orthogonal if each block taken independently is orthogonal. Same goes for rectangular matrices. In conclusion we can described grouped convolution as a "batch" of smaller orthogonal convolutions.

    \subsection{Putting it all together}
        todo beware that it is the toeplitz matrices that must have monotonic dimensions, not the weight matrices.

    \subsection{SOC}

        \begin{theorem}[Explicit conv exponential]

            We can rewrite the convolution exponential as follows:

            \begin{align}
                & x + \frac{K*x}{1!} + \frac{K*K*x}{2!} + \dots \\
                = & \left(Id + K + \frac{K \mathbconv K}{2!} + \frac{K \mathbconv K \mathbconv K }{3!} + \dots \right) * x            
            \end{align}
        \end{theorem}
            Then we can apply one conv instead of n convs. Note that the resulting kernel is then larger that the original one. In theory, this could unlock large speedups, but the gain is limited in practice as the implementation of convolution layers is optimized for small kernels and large images \cite{ding2022scaling}. However as we perform only a single convolution, the activations are stored only once regardless of the number of exponential iterations. In practice, this unlocks larger batch sizes.

\section{Efficient implementation of our composite approach}

    Block convolution is a special type of convolution where the Hadamard product is replaced by a matrix product. To the best of our knowledge the only differentiable implementation is available in the implementation of BCOP \cite{li_preventing_2019}. However, since there is no cuda kernel available for block convolutions the authors relied on nested loops to construct the convolution and used the pytorch's matmul to perform matrix multiplication on GPU. Unfortunately this approach does not leverage the fact that the nested loops could be paralleled. Also, pytorch does not allow easily to parallelize cuda operators (that are already paralleled).

    \paragraph{leveraging 2D convolution to compute block convolution:}
    \red{Given two convolution kernels $A\in{K}_{c_o,c,l_1,l_2}$ and $B\in{K}_{c,c_i,k_1,k_2}$, the block convolution $R=A\mathbconv B\in{K}_{c_o,c_i,(k_1+l_1-1),(k_2+l_2-1)}$ can be implemented as proposed in \cite{bcop} by unrolling all the loops and explicit the full summation:}
    In order to efficiently implement this operation we can unroll all the loops and explicit the full summation:
    \[
        R_{i,j,x,y} = \sum_{i' \in 0}^{k-l-1}\sum_{j' \in 0}^{k-l-1}\sum_{x' \in 0}^{n}\sum_{y' \in 0}^{n} A_{i,j',x,y'} * B_{i-i',j-j',x',y}
    \]
    \red{
    \[
        R_{m,n,i,j} = \sum_{k \in 0}^{c-1}\sum_{i' \in 0}^{k-l-1}\sum_{j' \in 0}^{k-l-1} A_{m,k,i',j'} . B_{k,n,i-i',j-j'}
    \]
    }
    % By transposing dimensions in $A$ and $B$, we can turn this summation into
    \red{Inspired by \cite{wang_orthogonal_2020}, which aimed to compute $A\mathbconv A^T$ to proove orthogonality. We propose to replace the computation $A\mathbconv B$  by a convolution with zero padding between $A$ and $B^T$.}
    By re-ordering the summation, this operation can be re-written to use a 2D convolution at its core. While the formal definition of convolution only allows to perform the convolution. Transpose convolutions allow to properly handle the "full" padding being required. The depth and channel dimension can then be used to perform the matrix multiplication, which is thanks to a transposition in the second matrix such that the element-wise product corresponds to the matrix product (padding "valid" is used to ensure that no convolution is performed on the "depth" axis, since both the input and the kernel have the same length on this axis. The hole process is described in the fig\ref{fig:code}.

    \begin{figure}
        \centering
            \begin{verbatim}
def fast_matrix_conv(m1, m2, groups=1):
    # m1 is m*n*k1*k2
    # m2 is nb*m*l1*l2
    m, n, k1, k2 = m1.shape
    nb, mb, l1, l2 = m2.shape
    assert m == mb * groups
    # Rearrange m1 for conv
    m1 = m1.transpose(0, 1)  # n*m*k1*k2
    # Rearrange m2 for conv
    m2 = m2.flip(-2, -1)
    # Run conv, output shape nb*n*(k+l-1)*(k+l-1)
    r2 = torch.nn.functional.conv2d(m1, m2, 
           groups=groups, 
           padding=(l1 - 1, l2 - 1))
    # Rearrange result
    return r2.transpose(0, 1)  # n*nb*(k+l-1)*(k+l-1)
    \end{verbatim}
        \caption{Pytorch implementation of the algorithm. Tensorflow implementation differs only in the data format.}
        \label{fig:code}
    \end{figure}

    
    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{flash_bcop/figs/benchmark/bloc_conv_speed_cin.png}
        \caption{kernel size is fixed while number of channels is increased. The runtime for 100 operation is reported on log scale. The previous implementation is very insensitive to the number of channels since the cost of the matrix multiplication is negligible against the cost of the convolution.}
        \label{fig:timeit_cin}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{flash_bcop/figs/benchmark/bloc_conv_speed_k.png}
        \caption{number of channels is set to 16 whil kernel size in increased. The runtime for 100 operation is reported on log scale. This implementation scale better to larger kernel sizes.}
        \label{fig:timeit_cin}
    \end{figure}

    \subsection{Further parallelism}

        Although the bloc convolution is at the core of BCOP, it is not the only costly operation involved: the orthogonalization procedure is also very costly. In particular the algorithm require the orthogonalisation of $ 2k $ matrices of shape $ c_m \times  \frac{c_m}{2} $ plus a matrix $ c_i \times c_o $. The successive application of two orthogonalization is much more expensive than the orthogonalization of $ 2k + 1 $ matrices. As the shape of the matrices mismatch, one can wonder if the construction of a $ c_m \times c_m $ is possible using multiple $ c_m \times  \frac{c_m}{2} $ matrices. To do this, we extended the construction of orthogonal matrices by multiplying householder matrices. We follow the original approch but instead of constructing $c_m$ Householder matrices using $c_m$ normalized vectors, we use only 2 $ c_m \times \frac{c_m}{2} $ matrices: $ A_t = A_{t-1} ( I - 2 MM^t ) $ where M is an partially orthogonal matrix. 

        In the original paper, the authors depicted an iterative algorithm to construct the orthogonal kernel. However one can notice that since the bloc convolution operation is associative we can rearrange all products in order to represent the algorithm as an associative parallel scan. Then by running operations in parallel, we can reduce the time complexity from $ k $ to $ \log k $ steps.

        \begin{figure}
            \centering
            \includegraphics[width=\linewidth]{flash_bcop/figs/benchmark/bcop_global_time.png}
            \caption{This formalism greatly reduces the overhead induced by the reparametrization, making BCOP competitive in terms of runtime. Especially this implementation scale better to the various setting we can find in a network (various strides, kernel sizes, and number of input/output channels}
            \label{fig:bcop_global}
        \end{figure}
    
        \begin{figure}
            \centering
            % \includegraphics[width=\linewidth]{flash_bcop/figs/benchmark/bcop_time_vs_conv.png}
            \includegraphics[width=\linewidth]{flash_bcop/figs/benchmark/bcop_global_time_cin.png}
            \caption{In large-scale setting, the overhead induced by the trivialization gets absorbed by the cost of the convolution, making this implementation competitive with standard convolutions. Also, this approach performs real striding: where the convolution get more efficient when striding is enabled (old implementation used emulated striding, that makes the convolution less efficient)}
            \label{fig:bcop_vs_conv}
        \end{figure}

\section{Evaluation of singular value and expressiveness}

    All code was unit tested with 1k test with coverage 89\%.

    \paragraph{Quick method:} spectral product of sub convolutions. OK if 1-lipschitz otherwise not precise (non alignment of eigen vectors)

    \paragraph{Exact approach SVD of the toelplitz matrix using impulse response} Ran extensive testing over configurations of channels stride, groups for both conv and convtranspose.

    \paragraph{Expressiveness testing}



\section{Applications}

    
\section{Application and expressiveness}

    \input{flash_bcop/tables/resnet50_overhead}

    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{flash_bcop/figs/robustness/pareto_robustness_cifar10_v3.png}
        \caption{Caption}
        \label{fig:enter-label}
    \end{figure}

\section{List of conducted experiments}

\paragraph{speed/ memory efficiency/expressiveness}

\begin{itemize}
    \item new bloc operator vs old bloc operator
    \item old layer vs new layer (func of nb channels, and as a func of kernel size)
    \item speed and memory resnet34 imagenet
\end{itemize}

\paragraph{robustness}
\begin{itemize}
    \item cifar10 non-robust: custom architecture, 93\% accuracy
    \item cifar10 robust: simple arch, competitive results 64\% VRA
    \item Imagenet non-robust: custom architecture 70\% accuracy
    \item Imagenet robust: simple arch, 42\% val acc, 26\% VRA.
\end{itemize}

\paragraph{TRaining dynamics}

\begin{itemize}
    \item very deep network: it trains but is very slow to converge
    \item vgg-250: tried it on imagenet, but it is veeeeeeeeery slooooooooooow
\end{itemize}

\paragraph{WGAN}

\begin{itemize}
    \item Starting from a tutorial notebook, trained a WGAN on cifar10, kinda ok (no numerical evaluation)
    \item Attempt to push the notebook to imagenet, seems to work (but data augmentation gives poor images)
    \item \textbf{TODO} test BiG-Gan repo on imagenet ?
\end{itemize}

\paragraph{Normalizing flows}

\textbf{TODO}

\paragraph{Semantic segmentation / UNets}

\textbf{TODO}


\section{Limitations and future works}

    We do not address the original expressiveness issue of BCOP, SC-Fac claims to solve it but restrict themselves to separable convolutions. We mitigate those with architectural tricks: channel increase, larger kernel size, larger networks.
    We investigate the roots of these issues and found that the resolution of this problem is deep enough to deserve its own line of work.

\section{Checklist}

    \begin{itemize}
        \item Add channel change + stride support to SOC + Cayley
        \item find a way to make the module.compile() to work
        \item implement and benchmark Gramm
        \item benchmark full training (time + memory)
        \item train a net on imagenet
        \item implement a unet on segmentation tasks
    \end{itemize}

    % \paragraph{How to sell this work ?} Here are the main thoughts about how to sell this work:
    % \begin{itemize}
    %     \item robustness benchmarks are tough to beat on cifar10/100 (To beat: 82.1\% clean 70.1\% VRA)
    %     \item training a network a network on imagenet is accessible: 1 concurrent only (to beat: 45\% clean, 35.0\% VRA)
    %     \item Explore diffusion models?
    %     \item Provide a library, architectures and a pretrained imagenet backbone
    % \end{itemize}


==> flash_bcop/tables/arch_desc_cifar10.tex <==



==> flash_bcop/tables/imgnet_arch.tex <==
% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|}
%         \hline
%         \textbf{Metric} & \textbf{BCOP\_new} & \textbf{Conv2D} \\
%         \hline
%         Max Train Memory (GB) & 21.566 & 18.340 \\
%         % \hline
%         Max Test Memory (GB) & 3.457 & 3.387 \\
%         % \hline
%         Train Mean & 1.008 & 0.706 \\
%         % \hline
%         Train Std Dev & 0.003 & 0.005 \\
%         % \hline
%         Test Cached Mean & 0.148 & 0.140 \\
%         % \hline
%         Test Cached Std Dev & 0.007 & 0.009 \\
%         % \hline
%         Test Caching Time & 0.084 & -0.078 \\
%         \hline
%     \end{tabular}
%     \caption{Comparison of BCOP\_new and Conv2D}
%     \label{tab:comparison}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|cccc}
%         \hline
%         \textbf{Model} & \textbf{Train Mem (GB)} & \textbf{Test Mem (GB)} & \textbf{Train time (s)} & \textbf{ Test time (s)} \\
%         \hline
%         BCOP\_new & 21.566 & 3.457 & 1.008 (0.003) & 0.148 (0.007) \\
%         \hline
%         Conv2D & 18.340 & 3.387 & 0.706 (0.005) & 0.140 (0.009) \\
%         \hline
%     \end{tabular}
%     \caption{Comparison of BCOP\_new and Conv2D}
%     \label{tab:comparison}
% \end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{c|cc}
        \hline
         & \textbf{BCOP\_new} & \textbf{Conv2D} \\
        \hline
        Train time (s) & 1.008 (0.003) & 0.706 (0.005) \\
        Train Mem (GB) & 21.566 & 18.340 \\
        Test time (s) & 0.148 (0.007) & 0.140 (0.009) \\
        Test Mem (GB) & 3.457 & 3.387 \\
    \end{tabular}
    \caption{With only a 1.42x train time overhead and a 1.17x train memory overhead, our implementation achieves competitive results on Imagenet. These numbers are computed on a realistic architecture that reaches 67\% validation accuracy. Experiments were run on an RTX-4090 consumer GPU}
    \label{tab:comparison}
\end{table}


==> flash_bcop/tables/methods_qualification_and_scaling.tex <==
\begin{figure*}[ht]
    \centering
    \begin{minipage}[t]{0.75\textwidth}  % Left half for the table
        \centering
        \resizebox{\textwidth}{!}{  % Scale table to fit within half the page width
            \begin{tabular}{lcp{18mm}p{14mm}p{15mm}p{10mm}p{16mm}c} 
                \textbf{Method} & \textbf{Orthogonal} & \textbf{Equivalent Kernel Size} & \textbf{Code available} & \textbf{Change Channels} & \textbf{Stride} & \textbf{Conv Transpose} & \textbf{Groups} \\
                \hline 
                \textbf{BCOP} \cite{li_preventing_2019} & \cmark & k & \cmark & \cmark & $\capprox$ & \xmark & \xmark \\
                \textbf{SC-Fac} \cite{su_scaling-up_2021} & \cmark & k separable & \xmark & \cmark &  \cmark & ? & ? \\
                \textbf{ECO} \cite{yu_constructing_2021} & \cmark & $I_w \times I_h$ & \xmark & $\capprox$ & $\capprox$ & \xmark & \xmark \\
                \textbf{Cayley} \cite{trockman_orthogonalizing_2021} & \cmark & $I_w \times I_h$ & \cmark & $\capprox$ & $\capprox$ & $\capprox$ & \xmark \\
                \textbf{LOT} \cite{xu_lot_2023} & \cmark & $I_w \times I_h$ & \cmark & \cmark & $\capprox$ & \xmark & \xmark \\
                \textbf{ProjUNN-T} \cite{kiani_projunn_2022} & \cmark & $I_w \times I_h$ & \cmark & \xmark & \xmark & \xmark & \xmark \\
                \textbf{SLL} \cite{araujo_unified_2023} & \xmark & composed & \cmark & \xmark & \xmark & \xmark & \xmark \\
                \textbf{Sandwich} \cite{wang_direct_2023} & \xmark & composed & \cmark & $\capprox$ & $\capprox$ & \xmark & \xmark \\
                \textbf{SOC} \cite{singla_skew_2021} & \cmark & $k + (n\frac{k}{2})$ & \cmark & $\capprox$ & $\capprox$ & \xmark & \xmark \\
                \hline
                \textbf{Our Method} & \cmark & k & \cmark & \cmark & \cmark & \cmark & \cmark \\
            \end{tabular}
        }
    \end{minipage}%
    \hfill
    \begin{minipage}[t]{0.25\textwidth}  % Right half for the plot
        \centering
        \includegraphics[width=\textwidth]{flash_bcop/figs/benchmark/bcop_global_time_new.png}
    \end{minipage}
    \caption{Comparison of orthogonal convolution methods and performance plot of our proposed method versus state-of-the-art methods. A check mark (\cmark) indicates full support for the feature, a cross mark (\xmark) indicates lack of support, and an approximate symbol ($\approx$) indicates partial support (emulation). Here, $k$ denotes the kernel size, and $I_w \times I_h$ represents the input dimensions.}
    \label{fig:comparison_and_performance}
\end{figure*}

